VILA$^2$: VILA Augmented VILA

While visual language model architectures and training infrastructures advance rapidly, data curation remains under-explored where quantity and quality become a bottleneck. Existing work either crawls extra Internet data with a loose guarantee of quality or distills from black-box proprietary models, e.g., GPT-4V / Gemini that are API frequency and performance bounded. This work enables a VLM to improve itself via data enhancement, exploiting its generative nature. We introduce a simple yet effective VLM augmentation scheme that includes a self-augment step and a specialist-augment step to iteratively improve data quality and hence, model performance. In the self-augment step, the instruction-finetuned VLM recaptions its pretraining caption datasets and then retrains from scratch leveraging refined data. Without any expensive human-in-the-loop annotation, we observe improvements in data quality and downstream accuracy boosts with three self-augmentation rounds -- a viable free lunch to the current VLM training recipe. When self-augmentation saturates, we augment the caption diversity by leveraging specialty skills picked up from instruction finetuning. We finetune VLM specialists from the self-augmented VLM with domain-specific experts, including spatial, grounding, and OCR, to fuse task-aware synthetic data into the pretraining stage. Data quality improvements and hallucination reductions are cross-checked by VLM (GPT-4V, Gemini) and human judges. Combining self-augmentation and specialist-augmented training, VILA$^2$ consistently improves the accuracy on a wide range of benchmarks over the prior art, producing a reusable pretraining dataset that is 300x more cost-efficient than human labeling.

==> tables/prompt_ablation.tex <==
% \begin{table}[]
% \begin{tcolorbox}[rounded corners=northeast]
% \centering
% \includegraphics[width=0.8\linewidth]{figures/caption_comparison.png}
% \end{tcolorbox}
% \caption{Place holder (sharegpt4v-style) for comparison, might use VILA1.0 Figure 6. style}
% \end{table}

\begin{table}[]
% \setlength{\fboxrule}{1pt}
\begin{tcolorbox}[rounded corners=northeast]
\begin{multicols}{2}
\small
\begin{minipage}[c][6cm][b]{10em}
% \begin{center}
\includegraphics[width=0.65\linewidth]{figures/prompt_example.jpg}
% \end{center}

\texttt{"<image> \#\#\# Short Description:}

\{origin text\}

\texttt{\#\#\# Long Description:}

\{re-captioned text\}\texttt{"}
\\[6pt]
(a). Concat Template 
\end{minipage}
\columnbreak
\footnotesize
\begin{minipage}[c][6cm][b]{30em}

\textbf{Simple Prompt}:

\texttt{"<image> Describe the image briefly."}

\textbf{Long Prompt v1}:

\texttt{"<image> Describe the image in details."}

\textbf{Long Prompt v2}:

\texttt{"<image> Elaborate on the visual and narrative elements of the image in detail."}

\textbf{Long Prompt v3}:

\texttt{"<image> Instead of describing the imaginary content, only describing the content one can determine confidently from the image. Do not describe the contents by itemizing them in list form. Minimize aesthetic descriptions as much as possible."}

\textbf{Mixed}: Random selection from v1 to v3.
\\
\begin{center}
    (b). Prompt Choices for Long Description
\end{center}
\end{minipage}
\end{multicols}
\end{tcolorbox}
\caption{Training template and prompt choices for self-augmenting. \ligeng{move to Method}}
\vspace{10pt}
\label{tab:prompt_ablation}
\end{table}

==> tables/ratio_comparison.tex <==
\begin{table*}[h]
\setlength{\tabcolsep}{3pt}
\centering
\scalebox{0.95}{
\begin{tabular}{lrrrrrrrrrrrr}\toprule
&GQA &LlavaBench &POPE &SCIENCE &SCIENCE-IMG &SEED &SEED-Image &MMMU\_VAL &MMVET &TextVQA &MME \\ \midrule
Baseline &62.37 &68.40 &0.84 &68.40 &68.10 &61.14 &69.00 &0.338 &34.50 &61.57 &1491.00 \\ \midrule
re-caption only &61.97 &69.40 &0.81 &68.89 &69.17 & & & & & & \\
re-caption + original &63.47 &72.20 &0.89 &71.46 &72.14 &62.50 &70.35 &0.352 &34.90 &63.54 &1510.20 \\
\bottomrule
\end{tabular}
}
\caption{
     Ablations on different mixing ratio between original data and re-captioned data. 
}
\vspace{5pt}
\label{tab:iteration_rounds}
\end{table*}

==> tables/rebuttal_sota_comparison.tex <==
% \begin{table*}[t]
% \setlength{\tabcolsep}{3pt}
% \centering
% \scalebox{0.63}{
% % \begin{tabular}{l l p{5mm}p{7mm}p{7mm} | p{8mm}p{8mm}p{8mm}p{8mm}p{8mm} | p{8mm}p{8mm}p{8mm} p{9mm} p{8mm} p{9mm} l }
% \begin{tabular}{l llll | lllll | llllll }
% \toprule
% Method & LLM & Res. & PT & IT & VQA$^\text{v2}$ & GQA & VizWiz &  SQA$^\text{I}$ & VQA$^\text{T}$& MMB & MMB$^\text{CN}$ & SEED & LLaVA$^\text{W}$ & MM-Vet \\
% \midrule
% \rowcolor{black!10} \multicolumn{15}{l}{\textit{Low Input Image Reslution}}\\
% BLIP-2~\cite{li2023blip} & Vicuna-13B & 224 & 129M & -- & 41.0 & 41 & 19.6 & 61 & 42.5 &  -- & -- & 46.4 & 38.1 & 22.4 \\
% InstructBLIP~\cite{Dai2023InstructBLIP} & Vicuna-7B & 224 & 129M & 1.2M & -- & 49.2 & 34.5 & 60.5 & 50.1  & 36 & 23.7 & 53.4 & 60.9 & 26.2 \\
% InstructBLIP~\cite{Dai2023InstructBLIP} & Vicuna-13B & 224 & 129M & 1.2M & -- & 49.5 & 33.4 & 63.1 & 50.7 & -- & -- & -- & 58.2 & 25.6 \\
% % IDEFICS-9B~\cite{idefics} & LLaMA-7B & 224 & 353M & 1M & 50.9 & 38.4 & -- & 25.9 & -- & 48.2 & 25.2 & -- & -- & -- \\
% % IDEFICS2-8B & Mistral-7B-v0.1 & 980 & & & & & & & & & & & & & \\
% Qwen-VL~\cite{bai2023qwen} & Qwen-7B & 448 & 1.4B & 50M & 78.8 & 59.3 & 35.2& 67.1 & 63.8 & 38.2 & 7.4 & 56.3 & -- & -- \\
% Qwen-VL-Chat~\cite{bai2023qwen} & Qwen-7B & 448 & 1.4B & 50M & 78.2 & 57.5 & 38.9 & 68.2 & 61.5 & 60.6 & 56.7 & 58.2 & -- & -- \\
% % \midrule
% % DeepSeek-VL & DeepSeek-LLM-7B & 1024 &  \\
% % LLaVA-NeXT-7B & Vicuna-1.5-7B & 672 & 0.7M & 0.8M & 81.8 & 64.2 & 70.1 & 64.9 & 86.5 & 67.4 & -- & 70.2 & 72.3 & 43.9\\
% % LLaVA-NeXT-13B & Vicuna-1.5-13B & 672 & 0.7M & 0.8M & 82.8 & 65.4 & 73.6 & 67.1 & 86.7 & 1519.3 & 70.0 & -- & 71.9 & 72.3 & 48.4\\
% LLaVA-1.5~\cite{liu2023improved} & Vicuna-1.5-7B & 336 & 0.6M & 0.7M & 78.5 & 62.0 & 50.0 & 66.8 & 58.2 & 64.3 & 58.3 & 58.6 & 63.4 & 30.5 \\ 
% LLaVA-1.5~\cite{liu2023improved} & Vicuna-1.5-13B & 336 & 0.6M & 0.7M & 80.0 & 63.3 & 53.6 & 71.6 & 61.3 & 67.7 & 63.6 & 61.6 & 70.7 & 35.4 \\
% % VILA-7B & Vicuna-1.5-7B & 672 & 50M & 0.8M & & & & & & & & & & &\\
% % VILA-13B & Vicuna-1.5-13B & 672 & 50M & 0.8M & & & & & & & & & & &\\

% % \midrule
% % OLD MODEL & Llama-2-7B & 336 & 50M & 1M & & 62.0 &b & 68.2 & 64.4 & 86.4 & f& 70.3 &h & & 69.7 & 38.3 \\
% % \rowcolor{black!10}
% % llama2-7b-clip336-mmc4sub+coyo-finetune-llava15+vflan-nosqa-linear-e1-nose-run2
% % VILA-7B & Llama-2-7B & 336 & 50M & 1M & 79.9$^*$  & \underline{62.3}$^*$ & \underline{57.8} & 68.2 & \underline{64.4} & \underline{85.5} & \underline{1533.0} & \underline{68.9} & 61.7 & 61.1 & 69.7 & 34.9 \\
% % \rowcolor{black!10}
% % llama2-13b-clip336-mmc4sub+coyo-finetune-llava15+vflan-nosqa-linearclip-e1-nose-run2
% % VILA-7B~\cite{lin2024vila} & Vicuna-1.5-7B & 336 & 50M & 1M & 79.9$^*$ & 62.3$^*$ & 68.2 & 64.4 &  85.5 & 68.9 & 61.7 & 61.1 & 69.7 & 34.9 & \\

% VILA-7B~\cite{lin2024vila} & Llama-2-7B & 336 & 50M & 1M & 79.9 & 62.3 & 57.8 & 68.2 & 64.4& 68.9 & 61.7 & 61.1 & 69.7 & 34.9 \\
% VILA-13B~\cite{lin2024vila} & Llama-2-13B & 336 & 50M & 1M & 80.8 & 63.3 & 60.6 & 73.7 & 66.6 & 70.3 & 64.3 & 62.8 & 73.0 & 38.8 \\
% % \methodshort & Llama-2-7B & 448 & 50M & 1M \\
% % \methodshort & Llama-2-13B & 448 & 50M & 1M & \\
% % \midrule \midrule
% % VILA-7B & Llama-2-7B & 336 & 50M & 1M &80.6$^*$ & 63.2$^*$ & 62.4 & 73.1 & 65.3 & 84.8 & 1556.5 & 70.8 & 65.4 & 61.4 & \textcolor{mydarkgreen}{78.4} & \textcolor{mydarkgreen}{45.7} \\
% % LLaVA-NeXT-7B & Vicuna-1.5-7B & 672 & 0.7M & 0.8M & 81.8 & 64.2 & 70.1 & 64.9 & 86.5 & 67.4 & -- & 70.2 & 72.3 & 43.9\\
% % VILA-7B & Vicuna-1.5-7B & 384 & 50M+7.5M & 4.9M & 79.9$^*$ & 62.3$^*$ & 68.2 & 64.4 &  85.5 & 68.9 & 61.7 & 61.1 & 69.7 & 34.9 & \\
% % \methodshort-7B (ours) & Vicuna-1.5-7B & 384 & 50M+7.5M & 4.9M & 82.0$^*$ & 63.2$^*$ & 87.0$^*$ & 64.9 &  86.6 & 75.3 & 66.2 & 64.4 & 74.3 & 38.5 & \\
% \rowcolor{mydarkgreen!10}\methodshort-8B (ours) & Llama-3-8B & 384+S2 & 51M & 6.5M & \ul{82.9} & 64.1 & \textbf{64.3} & \textbf{87.6} & \textbf{73.4} & \textbf{76.6} & \textbf{71.7} & \ul{66.1} & \textbf{86.6} & \textbf{50.0} \\
% \rowcolor{mydarkgreen!10}\methodshort-13B (ours) & Llama-2-13B & 384+S2 & 51M & 6.5M & \textbf{83.2} & 64.1 & \ul{61.3} & \ul{85.8} & \ul{72.1} & \ul{75.3} & \ul{68.4} & \textbf{66.2} & \ul{84.0} & \ul{46.4} \\
% \rowcolor{black!10} \multicolumn{15}{l}{\textit{High Input Image Reslution}}\\
% LLaVA-NeXT-8B~\cite{liu2024llavanext} & Llama-3-8B & 672 & & & -- & \textbf{65.2} & -- & 72.8 & 64.6 & 72.1 & -- & -- & 80.1 & -- \\
% Mini-Gemini-HD-8B~\cite{li2024minigeminiminingpotentialmultimodality} & Llama-3-8B & 1536 & & & -- & \ul{64.5} & -- & 75.1 & 70.2 & 72.7 & -- & -- & -- & -- \\
% Cambrian-1-8B & Llama-3-8B & 1024 & & & -- & 64.6 & 80.4 & 71.7 & -- & 75.9 & -- & - & -- & -- \\
% % \rowcolor{black!10} \methodshort-7B (ours) & Vicuna-1.5-7B & 384 & 50M+7.5M & 4.9M & 82.0$^*$ & 63.2$^*$ & 87.0$^*$ & 64.9 &  86.6 & 75.3 & 66.2 & 64.4 & 74.3 & 38.5 & \\
% % \rowcolor{black!10} \methodshort-13B (ours) & Vicuna-1.5-13B & 384 & 51M+7.5M & 4.9M & \textbf{82.5}$^*$ & \textbf{64.8}$^*$ & \textbf{89.0}$^*$ & \textbf{67.0} & \ul{85.6} & \textbf{75.6} & \textbf{68.0} & \textbf{64.5} & \ul{72.5} & \textbf{45.4} \\

% % LLaVA-NeXT-7B & Vicuna-1.5-7B & 672 & 0.7M & 0.8M & 81.8$^*$ & 64.2$^*$ & 70.1 & 64.9 & 86.5 & 67.4 & -- & 70.2 & 72.3 & 43.9\\

% \bottomrule
% \end{tabular}
% }
% \caption{
% Comparison with state-of-the-art methods on 10 visual-language benchmarks. Our models consistently improve VILA under a head-to-head comparison, using the same prompts and the same base LLM (Vicuna-1.5 is based on Llama-2), showing the effectiveness of enhanced pretraining data quality. $^*$The training images of the datasets are observed during training. We mark the best performance \textbf{bold} and the second-best \underline{underlined}.  
% }
% \vspace{5pt}
% \label{tab:sota_comparison}
% \end{table*}





\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\centering
\scalebox{0.70}{
\begin{tabular}{l ll | lllll | lllll }
\toprule
Method & LLM & Res. & VQA$^\text{v2}$ & GQA & VizWiz &  SQA$^\text{I}$ & VQA$^\text{T}$& MMB & MMB$^\text{CN}$ & SEED & LLaVA$^\text{W}$ & MM-Vet \\
\midrule
VILA-7B & Llama 2-7B & 336& 79.9 & 62.3 & 57.8 & 68.2 & 64.4& 68.9 & 61.7 & 61.1 & 69.7 & 34.9 \\
VILA-13B & Llama 2-13B & 336& \ul{80.8} & 63.3 & \ul{60.6} & 73.7 & 66.6 & 70.3 & \ul{64.3} & \ul{62.8} & 73.0 & \ul{38.8} \\

% \rowcolor{black!10} \multicolumn{13}{l}{\textit{High Input Image Reslution}}\\
LLaVA-NeXT-8B & Llama 3-8B & 672 & -- & \textbf{65.2} & -- & 72.8 & 64.6 & 72.1 & -- & -- & \ul{80.1} & -- \\
% Idefics2-8B~\cite{laurençon2024mattersbuildingvisionlanguagemodels} & Llama 3-8B & 980 & 81.2 & -- & -- & -- & \ul{73.0} & \textbf{76.7} & -- & -- & -- & -- \\
Cambrian-1-8B & Llama 3-8B & 1024 & -- & \ul{64.6} & -- & \ul{80.4} & \ul{71.7} & \ul{75.9} & -- & -- & -- & -- \\
Mini-Gemini-HD-8B & Llama 3-8B & 1536 & -- & 64.5 & -- & 75.1 & 70.2 & 72.7 & -- & -- & -- & -- \\
% LLaVA-NeXT-7B & Vicuna-1.5-7B & 672 & 0.7M & 0.8M & 81.8$^*$ & 64.2$^*$ & 70.1 & 64.9 & 86.5 & 67.4 & -- & 70.2 & 72.3 & 43.9\\
\midrule
\rowcolor{myopen}\methodshort-8B (ours) & Llama 3-8B & 384& \textbf{82.9} & 64.1 & \textbf{64.3} & \textbf{87.6} & \textbf{73.4} & \textbf{76.6} & \textbf{71.7} & \textbf{66.1} & \textbf{86.6} & \textbf{50.0} \\
% \rowcolor{myopen}\methodshort-34B (ours\yunhao{ntd}) & Yi-34B & 448& 85.1 & 64.7 & 62.2  & 93.2 & 75.9 & 83.9 & 82.9 & 77.0 & 93.6 & 53.4 \\
\bottomrule
\end{tabular}
}
\caption{
Comparison with state-of-the-art methods on 10 visual-language benchmarks. Our models consistently improve VILA under a head-to-head comparison, using the same prompts and the same base LLM, showing the effectiveness of enhanced pretraining data quality. We mark the best performance \textbf{bold} and the second-best \underline{underlined}.
% \ligeng{@yunhao check bold and underline}
}
% \vspace{5pt}
\label{tab:sota_comparison}
\end{table*}




==> tables/rebuttal_specialist_comparison.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\centering

\scalebox{0.80}{
\begin{tabular}{l|llllllll}\toprule
&VQA$^\text{v2}$&GQA &VQA$^\text{T}$ & POPE &SEED-I& MME &MM-Vet&MMMU (T) \\ \midrule
\rowcolor{black!10} \multicolumn{9}{l}{\textit{Pretrain Data: 10\%\ MMC4-core+10\%\ COYO-25M+ShareGPT4V-Pretrain}}\\
Original Caption& 81.4\phantom{\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.0}}} & 63.8\phantom{\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.0}}}& 65.2\phantom{\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.0}}} & 85.5\phantom{\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.0}}} & 70.6\phantom{\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.0}}} & 1472.5\phantom{\textsubscript{\textcolor{mydarkgreen}{$\uparrow$00.0}}} & 34.0\phantom{\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.0}}}& 31.8\phantom{\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.0}}} \\
+ Spatial Specialist     & \textbf{81.9}\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.5}} & \textbf{64.1}\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.3}} & \textbf{66.0}\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.8}} & 85.9\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.4}} & 71.8\textsubscript{\textcolor{mydarkgreen}{$\uparrow$1.2}} & 1476.5\textsubscript{\textcolor{mydarkgreen}{$\uparrow$4.0}}\phantom{\textsubscript{0}} & 36.7\textsubscript{\textcolor{mydarkgreen}{$\uparrow$2.7}} & 32.5\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.7}} \\
 + OCR Specialist     & 81.8\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.4}} & 64.0\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.2}} &  65.3\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.1}} & 86.4\ \textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.9}} & \textbf{72.1}\textsubscript{\textcolor{mydarkgreen}{$\uparrow$1.5}} & 1500.2\textsubscript{\textcolor{mydarkgreen}{$\uparrow$27.7}} & 34.3\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.3}} & 32.1\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.3}} \\
 + Grounding Specialist     & 81.8\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.4}} & 64.0\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.2}} &  65.1\textsubscript{\textcolor{mydarkred}{$\downarrow$0.1}} & \textbf{86.7}\textsubscript{\textcolor{mydarkgreen}{$\uparrow$1.2}} & 71.0\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.4}} & \textbf{1536.4}\textsubscript{\textcolor{mydarkgreen}{$\uparrow$63.9}} & \textbf{37.5}\textsubscript{\textcolor{mydarkgreen}{$\uparrow$3.5}} & \textbf{32.6}\textsubscript{\textcolor{mydarkgreen}{$\uparrow$0.8}} \\ \midrule
\rowcolor{black!10} \multicolumn{9}{l}{\textit{Pretrain Data: MMC4-core+COYO-25M+ShareGPT4V-Pretrain}}\\
Original Caption & 82.2 & 63.9 & 66.7 & \textbf{86.5} & 71.2 & 1518.2 & 42.6 & 33.4 \\ 
+ All 3 Specialist & \textbf{83.0}\textsubscript{\textcolor{mydarkgreen}{+0.8}} & \textbf{64.7}\textsubscript{\textcolor{mydarkgreen}{+0.8}} & \textbf{70.9}\textsubscript{\textcolor{mydarkgreen}{+4.2}} & 86.4\textsubscript{\textcolor{mydarkred}{-0.1}} & \textbf{74.0}\textsubscript{\textcolor{mydarkgreen}{+2.8}} & \textbf{1656.2} \textsubscript{\textcolor{mydarkgreen}{+142} }& \textbf{44.7} \textsubscript{\textcolor{mydarkgreen}{+2.1}} & \textbf{35.8}\textsubscript{\textcolor{mydarkgreen}{+2.4}} \\ 
% \rowcolor{green!10} Improvement &  & \textcolor{mydarkgreen}{+0.8} & \textcolor{mydarkgreen}{+4.2} & \textcolor{mydarkred}{-0.1} & \textcolor{mydarkgreen}{+2.8} & \textcolor{mydarkgreen}{+142} & \textcolor{mydarkgreen}{+2.1} & \textcolor{mydarkgreen}{+2.4} \\ 
% \midrule
% \rowcolor{black!10}  \vila{3}+Specialist 
% & \textbf{81.1} & 62.8 & \textbf{72.9} & \textbf{65.0} & \textbf{85.0} & 71.4 & \textbf{37.1} & \textbf{36.8 }\\
\bottomrule
\end{tabular}
}
% \vspace{-1mm}
\caption{
    Effectiveness of the data re-captioned by  specialists:  
    % `Spatial' for the \textit{Scene Relations Understanding} specialist, `Textual' for the \textit{Textual Content Recognition} specialist, and `Grounded' for the \textit{Grounded Narration} specialist. Specialists-annotated data are curated as QA pairs and concatenated to the original caption. 
    We mark the best performance with \textbf{bold}. The results in the same block are trained with different pretraining data but the same SFT data. 
    Specialists-annotated data consistently improves  on both 10\% and 100\% pretraining setting.
    % All models are based on Llama 3-8B-Instruct.
    % Models are pre-trained with 2.5M (specialist-captioned) COYO images, 0.6M MMC4-core images, and 1M ShareGPT4V-Pretrain images.
}
\label{tab:specialist_comparison}
\end{table*}


==> tables/specialist_effectiveness.tex <==
% \begin{table*}[t]
% \setlength{\tabcolsep}{3pt}
% \centering

% \scalebox{0.8}{
% \begin{tabular}{ll|ccc|ccc|cc|c}\toprule
% Model & Size &\multicolumn{3}{c}{RefCOCO}&\multicolumn{3}{c}{RefCOCO+}&\multicolumn{2}{c}{RefCOCOg}& \\
% && val & testA & testB & val & testA & testB &val &test &Avg.\\ \midrule

% Cube-LLM & 7B & 90.9 & 92.6 & 87.9 & 83.9 & 89.2 & 77.4 & 86.6 & 87.2 & 87.0 \\
% \methodshort (Grounding Specialist)& 8B & 91.0 & 94.1 & 87.6 & 86.0 & 90.4 & 79.2 & 87.8 & 88.6 & 88.1 \\ 
% \bottomrule
% \end{tabular}
% }
% % \vspace{-1mm}
% \caption{
%     Effectiveness of our grounding specialist.
% }
% \label{tab:grounding_specialist}
% \end{table*}


==> tables/specialty_acquisition.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\centering

\scalebox{0.8}{
\begin{tabular}{l|cccccccc}\toprule
&VQA$^\text{v2}$&GQA &SQA &VQA$^\text{T}$ & POPE &LLaVA$^\text{W}$& MM-Vet&MMMU \\ \midrule
\vila{0} - Baseline & 79.6 & 62.4&68.4&61.6&84.2&68.4&34.5&33.8 \\ \midrule
\vila{1} &80.0&63.2&71.0 &62.5 &84.6 &72.2 &34.8 &\ul{35.8} \\
\vila{2} &\ul{80.8}&\textbf{63.5}& {71.5} & 63.5&{84.7} &71.2& 34.9 &35.2 \\
\rowcolor{black!10}  \vila{3} & 80.7 &\textbf{63.5}&\ul{71.5}& \ul{63.7} & 84.5 & \textbf{72.3} & {35.5} & {35.5} \\
\vila{4} & {80.7} & 63.4&71.2 & {63.6} & \textbf{85.0} &\textbf{72.3} & \ul{35.5} & 35.0 \\ 
\midrule
\bottomrule
\end{tabular}
}
% \vspace{-1mm}
\caption{specialty acquisition }
\label{tab:specialty_acquisition}
\end{table*}


==> tables/state_of_the_art.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{3pt}
\centering
\scalebox{0.75}{
\begin{tabular}{lc | llll | llll | lll }
\toprule
Method& \# Vis Tok. & VQA$^\text{v2}$ & VizWiz & GQA & SQA$^\text{I}$ & VQA$^\text{T}$ & POPE & MMB & MMB$^\text{CN}$ & SEED & LLaVA$^\text{W}$ & MM-Vet \\
\midrule
\rowcolor{black!10} \multicolumn{13}{l}{\textit{Base LLM: Llama-3-Ins-8B}}\\
Mini-Gemini-HD-8B & 2880& - & - & 64.5 & 75.1 & 70.2 & - & 72.7 & - & 73.2 & - & - \\
LLaVA-NeXT-8B & 2880& - & - & \textbf{65.2} & 72.8 & 64.6 & - & 72.1 & - & 72.7 & 80.1 & - \\
Cambrian-1-8B & 576 & - & - & 64.6 & 80.4 & 71.7 & - & 75.9 & - & 74.7 & - & - \\
VILA1.5-8B & 196 & 80.9 & 58.7 & 61.9 & 79.9 & 66.3 & 84.4 & 72.3 & 66.2 & 71.1 & 80.0 & 38.3 \\
\rowcolor{yellow!10}(neurips)\methodshort-7B & 196 & 82.0 & - & 63.2 & 87.0 & 64.9 & 86.6 & 75.3 & 66.2 & 64.4 & 74.3 & 38.5 \\
\rowcolor{yellow!10}(neurips)\methodshort-13B & 196 & 82.5 & - & 64.8 & 89.0 & 67.0 & 85.6 & 75.6 & 68.0 & 64.5 & 72.5 & 45.4 \\
\rowcolor{green!10} \methodshort-8B & \rowcolor{purple!10} 196 &\rowcolor{green!10} \textbf{83.0} & \textbf{63.7} & 64.3 & \textbf{87.6} & \textbf{73.1} & \textbf{86.7} & \textbf{77.9} & \textbf{71.2} & \textbf{74.7} & \textbf{84.7} & \textbf{46.8} \\
% \rowcolor{black!10} \multicolumn{13}{l}{\textit{Base LLM: Vicuna-1.5-13B}}\\
% Mini-Gemini-HD-13B & 2880& - & - & 63.7 & 71.9 & 70.2 & - & 68.6 & - & 70.6 & - & - \\
% LLaVA-NeXT-13B & 2880& - & - & - & - & - & - & - & - & - & - & - \\
% Cambrian-1-13B & 576 & - & - & - & - & - & - & - & - & - & - & - \\
% VILA1.5-13B & 196 & 82.8 & 62.6 & 64.3 & 80.1 & 65.0 & 86.3 & 74.9 & 66.3 & 72.6 & 80.8 & 44.3 \\
% \rowcolor{green!10} \methodshort-13B & \rowcolor{purple!10} 196 &\rowcolor{green!10} - & - & - & - & - & - & - & - & - & - & - \\
% \rowcolor{black!10} \multicolumn{13}{l}{\textit{Base LLM: Hermes2-Yi-34B}}\\
% Mini-Gemini-HD-34B & 2880& - & - & - & - & - & - & - & - & - & - & - \\
% LLaVA-NeXT-34B & 2880& - & - & - & - & - & - & - & - & - & - & - \\
% Cambrian-1-34B & 576 & - & - & - & - & - & - & - & - & - & - & - \\
% VILA1.5-34B & 196 & 84.3 & 62.2 & 64.6 & 87.2 & 73.2 & 88.2 & 82.4 & 80.2 & 75.8 & 81.3 & 53.0 \\
% \rowcolor{green!10} \methodshort-34B & \rowcolor{purple!10} 196 &\rowcolor{green!10}  - & - & - & - & - & - & - & - & - & - & - \\
\bottomrule
\end{tabular}
}
\caption{
Comparison with state-of-the-art methods on 11 visual-language benchmarks. Our models consistently improve VILA under a head-to-head comparison, using the same prompts and the same base LLM , showing the effectiveness of enhanced pretraining data quality We mark the best performance \textbf{bold}.
}
\vspace{5pt}
\label{tab:state_of_the_art}
\end{table*}

==> tables/vila2_benefits.tex <==
\begin{table*}[h]
\setlength{\tabcolsep}{3pt}
\centering

\scalebox{0.8}{
\begin{tabular}{ll|cccccccc}\toprule
& SFT &VQA$^\text{v2}$&GQA &VQA$^\text{T}$ & POPE &SEED-I& MME &MM-Vet&MMMU \\ \midrule
VILA1.5-8B (Simple)& 1.8M & 82.2 & 63.9 & 66.7 & 86.5 & 71.2 & 1518.2 & 42.6 & 33.4 \\ 
\methodshort-8B (Simple)& 1.8M & 83.0 & 64.7 & 70.9 & 86.4 & 74.0 & 1656.2 & 44.7 & 35.8 \\ 
\rowcolor{green!10}\methodshort Improvement& & \textcolor{mydarkgreen}{+0.8} & \textcolor{mydarkgreen}{+0.8} & \textcolor{mydarkgreen}{+4.2} & \textcolor{mydarkred}{-0.1} & \textcolor{mydarkgreen}{+2.8} & \textcolor{mydarkgreen}{+142} & \textcolor{mydarkgreen}{+2.1} & \textcolor{mydarkgreen}{+2.4} \\ 
VILA1.5-8B (All) & 5.9M & 82.6 & 64.1 & 70.8 & 86.4 & 65.6 & 1564.4 & 50.4 & 37.8 \\ 
\methodshort-8B (All) & 5.9M & 82.9 & 64.1 & 73.2 & 86.5 & 66.1 & 1594.6 & 50 & 38.3 \\ 
\rowcolor{green!10} \methodshort Improvement & & \textcolor{mydarkgreen}{+0.3} & \textcolor{mydarkgreen}{+0.0} & \textcolor{mydarkgreen}{+2.4} & \textcolor{mydarkgreen}{+0.1} & \textcolor{mydarkgreen}{+0.5} & \textcolor{mydarkgreen}{+30.2} & \textcolor{mydarkred}{-0.4} & \textcolor{mydarkgreen}{+0.5} \\ 
% VILA1.5-8B (All) & & & & & & & & \\ 
% \rowcolor{green!10} Gain (All) & & & & & & & & \\ 
% \midrule
% \rowcolor{black!10}  \vila{3}+Specialist 
% & \textbf{81.1} & 62.8 & \textbf{72.9} & \textbf{65.0} & \textbf{85.0} & 71.4 & \textbf{37.1} & \textbf{36.8 }\\
\bottomrule
\end{tabular}
}
% \vspace{-1mm}
\caption{
    Comparison of performance improvements from \methodshort with varying amounts of SFT data. While more high-quality SFT data generally enhances performance on most VQA benchmarks, the benefits of pretraining significantly diminish.
}
\label{tab:vila2_benefits}
\end{table*}

